SwitchOut: an Efficient Data Augmentation Algorithm for Neural Machine Translation

In this work, we examine methods for data augmentation for text-based tasks such as neural machine translation (NMT). We formulate the design of a data augmentation policy with desirable properties as an optimization problem, and derive a generic analytic solution. This solution not only subsumes some existing augmentation schemes, but also leads to an extremely simple data augmentation strategy for NMT: randomly replacing words in both the source sentence and the target sentence with other random words from their corresponding vocabularies. We name this method SwitchOut. Experiments on three translation datasets of different scales show that SwitchOut yields consistent improvements of about 0.5 BLEU, achieving better or comparable performances to strong alternatives such as word dropout (Sennrich et al., 2016a). Code to implement this method is included in the appendix.

==> related.tex <==
\section{\label{sec:related}Related Work}
Data augmentation for NMT is a longstanding challenge with a scarce body of literature. The most related work to ours is that of~\citet{nmt_data_augmentation}, which shows that data augmentation can improve NMT's performance on low-resource languages. Their technique swaps in pairs of source and target words, and requires a pre-trained language model and an alignment model to ensure that the augmented pairs of source-target sentences are semantically consistent and that such augmented pairs do not deviate too far from the training data. \sc~does not require such pre-trained models but has the benefits of being more efficient and easier to implement. % While we did not directly compare to this method due to its significantly increased complexity, by re-defining their method as a similarity function, it is likely that their method could also be implemented as a variant of our framework.

The idea of replacing the words in the text sequences has also been explored, \eg~by~\citet{seq2seq_semi} in learning a semi-supervised sequence-to-sequence model. However, they use a different distribution $\q$ on the augmented source sentences than ours, and optimize an auto-encoding objective. Since this objective is much easier to optimize, the effectiveness of the replacement of the source words is not clearly shown. From the perspective of Bayesian modeling,~\citet{variational_dropout_rnn} propose an alternative formulation of word dropout: replacing some words in the vocabulary with word embeddings that are filled with $0$'s. As shown in our experiments, \sc~delivers stronger results.

The theoretical framework of \sc~takes inspiration from~\citet{raml} in several ways. First, ~\citet{raml}~mentions that adding the entropy term to $J_\text{AUG}$ in~\eqref{eqn:data_aug} follows the entropy-regularized reinforcement learning objective. Second, we adopt the Hamming distance based importance sampling from \raml to derive an efficient algorithm. That said, in theory,~\raml~is a special case of our framework, as discussed in Section~\ref{sec:method}.

% ~\citet{raml} propose to minimize the KL divergence between: 1) an exponentiated payoff distribution over the target sentences and 2) the model's distribution. However, due to the intractable sampling process, the implementation of \raml~cannot support an exponentiated payoff distribution induced by arbitrary reward function. Instead,~\raml~resorts to importance sampling based on the Hamming distance that we discussed in Section~\ref{sec:method}. This makes~\raml~a special case of our framework, where $\tau_{x} \to \infty$,~\ie~there is no data augmentation on the source side.



